State space models vs. multi-step predictors in predictive control: Are state space models complicating safe data-driven designs?

This paper contrasts recursive state space models and direct multi-step predictors for linear predictive control. We provide a tutorial exposition for both model structures to solve the following problems: 1. stochastic optimal control; 2. system identification; 3. stochastic optimal control based on the estimated model. Throughout the paper, we provide detailed discussions of the benefits and limitations of these two model parametrizations for predictive control and highlight the relation to existing works. Additionally, we derive a novel (partially tight) constraint tightening for stochastic predictive control with parametric uncertainty in the multi-step predictor.

==> Literature_list.tex <==
%!TEX root = ./StateSpace.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  
 
\textbf{References (not yet used)}
\textbf{SysID}
\begin{itemize}
\item \cite{tsiamis2019finite} subspace, LS, hankel, bounds cross-correlation term; 
less-trivial arguments, general bounds with rate
\item \cite{gibson2005robust} expectation-maximisation;\\
iteratively make kalman that MLE based on estimates; resulting in a guaranteed improvement of the likelihood

\item \cite{umenberger2018maximum}: MLE; disturbances+noise using EM;
main additional contribution adding stability constraints using MM (minimizing upper bound instead of true)%: (with additional constraint)

\item \cite{tangirala2018principles}
\end{itemize}
\begin{itemize}
%\item OLd MPC with impulse response
%\begin{itemize}
%\item \cite{richalet1978model}: first industrial applications (process control) using impulse response\\
%also allows for easy estimation online (cf.~\cite{mayne2000constrained})
%\item \cite{cutler1980dynamic}: also early MPC industry; also use step response
%\item \cite{garcia1989model}: overview MPC; not needed
%\item \cite{lundstrom1995limitations}: limitation early approach: only considered output noise; not disturbances;
%modelling impulse/step response for long horizon increases number of parameters\\
%call to move  to state space models (with observers), to solve some of these issues
%\item standard MPC with state space today (at least in academia), cf. \cite{mayne2000constrained,rawlings2017model}   %grune2017nonlinear
%\end{itemize}
%\item Robustness in old impulse
%(cf. \cite[Sec.~4.1]{mayne2000constrained})\\
%\cite{zheng1993robust}: robust stabiliy in FIR; bound on impulse response (absolute/infinite-norm), min-max problems; (use directly in Section III.C)\\
%\cite{genceli1993robust,de1996robust}: also robust stability with bounds impulse response; less about constraints; more about stability
%but no min-max; so less relevant; more about offset-free\\
%\item Other convoluted prediction models in the literature:
%\begin{itemize}
%\item RAMPC using FIR~\cite{tanaskovic2014adaptive};% cf. also stochastic \cite{bujarbaruah2018adaptive};
%also for direct robustness handeling; without conservative over-approximations as in tube MPC
%\item Orthonormal basis functions (more general than FIR/impulse response; but keep parametrization benefits)\\
%\cite{heuberger1995generalized}: applicable to stable systems, requires fewer parameters the impulse response; easy to identify (no local minima); (basis can be constructed based on SVD of Hankel matrix); also to incorporate prior information in basis functions (e.g., rough location of poles)\\
%\cite{bachnas2015data}
%\cite{heirung2017dual} use for dual, by allowing for deterministic prediction of the Information matrix (cf. also \cite{soloperto2019dual}).
%(in comparison, with uncertain state space models; guaranteed lower bounds on PE are non-trivial, cf.~\cite[Sec.~3.4]{lu2021robust})\\
%similarly applicable to compute prob./robust reachable set directly.
%\item Multi-step prediction models\\
%\cite{terzi2018learning,terzi2018robust} (ECC18): identification and corresponding MPC\\
% journal \cite{terzi2019learning}: identification + RMPC; example shows better that one-step\\
%CDC19~\cite{salvador2019learning}: extend \cite{terzi2019learning} to MIMO  \\
%\cite{lauricella2020data}: only output noise; but keep parameteric error with LP\\%combine multiple multi-step predictors with intersection;\\
%\cite{terzi2022robust}: prove  that error bounds better than any one-step iterated (cf.~\cite[Thm.~1]{terzi2022robust}); also exploit bounds better using multi-rate (multi-step)\\ 
% use set-membership estimation for I/O with noise disturbances; \\
%show theoretically and numercally that directly using a estimated bound for a multi-step prediction is no worse than estimating a one-step bound and propagating %it over multiple steps 
%(however, the authors conservatively over-approximate the parametric model uncertainty as an additive term using compact region of operation, thus resulting in additional conservatism)\\
%also good reference regarding closed-loop issues; and middle ground 

%\item SPC~\cite{favoreel1999spc}: identify multi-step predictor/impulse response (which can be directly used in MPC); instead of first identifying a state space model\\%,kadali2003data
%DeepC~\cite{coulson2021distributionally,berberich2020data,dorfler2021bridging} jointly solve control and identification using implicit model based on Hankel matrices\\
% also for simple/direct robustification without propagating uncertainties~\cite{huang2021robust}\\ %coulson2021distributionally
%additional effect regarding direct and indirect is discussed here~\cite{dorfler2021bridging}, however, 
%We would like to note that when comparing DeePC with standard model-based MPC; the difference is not only attributable to the fact that a \textit{direct} data-driven design is used (cf.~\cite{dorfler2021bridging} for a detailed discussion on potential benefits); but also due to the fact that a convoluted prediction model is identified (as also done in Section~3.C) instead of a state space model.\\
%\cite{yin2021maximum}: Signal matrix model (Hankel matrix); only output noise; statistical ident with minimal prediction error~\cite{yin2021data}; requires observability matrix..%\\
%\cite{yin2021maximum_L4dc}: L4DC, less theory

%\item SLS~\cite{anderson2019system}: a method to  optimize feedback policies in a convex fashion by parametrizing the problem using convoluted maps (the closed-loop response); instead of directly using the state space model\\
%\cite{furieri2021near}: Behavioral InputOutput Parametrization (BIOP),  InputOutput Parametrization (IOP); also directly identifies $G$; similar to Section III.C\\
%data-driven SLS~\cite{xue2021data}: state, additive disturbances; no robust constraints\\
%
%This parametrization in terms of convoluted maps also allows for easier bounds to compute over-approximation of the reachable sets under parametric uncertainty, compare, e.g., \cite{bujarbaruah2020robust,chen2021system}.
%\cite{bujarbaruah2020robust} tightening directly uses |X|
%\cite{chen2021system}; SLS; good/reasonable bound; 
%Note that these approaches consider a parametric error in the state space, which is then over-approximated as a parametric error on the convoluted map $G$, before robust techniques similar to Section III.C can be applied.
 
 

 


%\item Nonlinear: \\
%KPC~\cite{maddalena2021kpc}: use multi-step prediciton to avoid propagating sets\\
%also kernel based with multi-step~\cite{thorpe2022data}\\
%volterra series~\cite{gruber2013computationally}; can solve min-max by using an efficient vertex enumeration;  (comparable to FIR)
%\end{itemize}
\item Robust MPC techniques; %specifically that can handle parametric uncertainty (resulting from Sys-ID)\\
%reachability with IQC (for fixed inputs)~\cite{seiler2019finite}; requires expensive LMIs and in general the IQC-parametrization over-approximates that parametric uncertainty, resulting in an over-approximation of the true reachable set. \\
% and such IQC techniques in MPC few results~\cite{schwenkel2021model}\\
%general tube methods~\cite[Sec.~5.5]{kouvaritakis2016model}\\
%multiplicative~\cite{fleming2014robust}, RAMPC (homethetic/general)~\cite{lorenzen2019robust,lu2021robust};\\
%however, drastically increased complexity~\cite[Table~1]{Koehler2019Adaptive} (even for small systems, $\#$ constraints/opt.-variables can increase by multiple-orders of magnitude); and still the methods are conservative, i.e., the fixed parametrization in the propagation results in (sometimes considerable) over-approximation of the reachable set\\
complexity issues can also be over-come by over-approximating constant additive bounds (cf.~\cite{falugi2013getting,bujarbaruah2021simple,wabersich2021nonlinear}), which, however, can significantly restrict performance
also \cite{wabersich2021probabilistic}?

 
%tube-based robust/stochatic MPC designs with guarantees regarding constraint satisfaction~\cite{}, however, largely limited to additive disturbance.
%On the other hand, Sys-ID under noise and disturbances results in a parametric error in the model; and over-approximations thereof as a uniformly bounded additive disturbances tend to be overly conservative. 

%\item Parameter estimation\\
%\cite{fogel1982value}
%\item SysID
%\cite{aastrom1971system}:
%Equ (35): Kalman filter results in i.i.d., disturbance in estimated state\\
%Section V: should I identify FIR or state?\\
%references[79-86]
%write ARX; then easy\\
%Example Section V: get corrolated disturbances $\Rightarrow$ usually get bias!\\
%solutions: \\
%repeated LS: higher order might deal with correlated\\
%generalized LS: correlation known (output of linear system driven by white noise);  
%rewrite linear system by "dividing" by this linear system to get a system driven by white noise;  corresponds to LS on a generalized error, which is filtered\\
% MLE: nonlinear in corrolation coefficients; resulting accuracy: \cite{aastrom1965automatic}:
%instrumental variables: multiply by matrix, s.t., expected value becomes zero\\
% Levin's method:
% tally principle\\

\end{itemize}


